AuxMix: Semi-Supervised Learning with Unconstrained Unlabeled Data

Semi-supervised learning (SSL) has seen great strides when labeled data is scarce but unlabeled data is abundant. Critically, most recent work assume that such unlabeled data is drawn from the same distribution as the labeled data. In this work, we show that state-of-the-art SSL algorithms suffer a degradation in performance in the presence of unlabeled auxiliary data that does not necessarily possess the same class distribution as the labeled set. We term this problem as Auxiliary-SSL and propose AuxMix, an algorithm that leverages self-supervised learning tasks to learn generic features in order to mask auxiliary data that are not semantically similar to the labeled set. We also propose to regularize learning by maximizing the predicted entropy for dissimilar auxiliary samples. We show an improvement of 5% over existing baselines on a ResNet-50 model when trained on CIFAR10 dataset with 4k labeled samples and all unlabeled data is drawn from the Tiny-ImageNet dataset. We report competitive results on several datasets and conduct ablation studies.

==> references_long.tex <==
@article{entmax-hinton-2017,
  author    = {Gabriel Pereyra and
               George Tucker and
               Jan Chorowski and
               Lukasz Kaiser and
               Geoffrey E. Hinton},
  title     = {Regularizing Neural Networks by Penalizing Confident Output Distributions},
  journal   = {CoRR},
  volume    = {abs/1701.06548},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.06548},
  archivePrefix = {arXiv},
  eprint    = {1701.06548},
  timestamp = {Mon, 13 Aug 2018 16:48:27 +0200},
}


@inproceedings{rotnet-2018,
  title={Unsupervised Representation Learning by Predicting Image Rotations},
  author={Gidaris, Spyros and Singh, Praveer and Komodakis, Nikos},
  booktitle={International Conference on Learning Representations},
  year={2018}
}



@article{fixmatch-2020,
  title={FixMatch: Simplifying Semi-Supervised Learning with Consistency and Confidence},
  author={Sohn, Kihyuk and Berthelot, David and Carlini, Nicholas and Zhang, Zizhao and Zhang, Han and Raffel, Colin A and Cubuk, Ekin Dogus and Kurakin, Alexey and Li, Chun-Liang},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}


@article{jing2020self,
  title={Self-supervised visual feature learning with deep neural networks: A survey},
  author={Jing, Longlong and Tian, Yingli},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2020},
  publisher={IEEE}
}

@article{randaug-2019,
  author    = {Ekin D. Cubuk and
               Barret Zoph and
               Jonathon Shlens and
               Quoc V. Le},
  title     = {RandAugment: Practical data augmentation with no separate search},
  journal   = {CoRR},
  volume    = {abs/1909.13719},
  year      = {2019},
  url       = {http://arxiv.org/abs/1909.13719},
  archivePrefix = {arXiv},
  eprint    = {1909.13719},
  timestamp = {Wed, 02 Oct 2019 13:04:08 +0200},
}

@article{meanteacher-2017,
  author    = {Antti Tarvainen and
               Harri Valpola},
  title     = {Weight-averaged consistency targets improve semi-supervised deep learning
               results},
  journal   = {CoRR},
  volume    = {abs/1703.01780},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.01780},
  archivePrefix = {arXiv},
  eprint    = {1703.01780},
  timestamp = {Mon, 13 Aug 2018 16:49:09 +0200},
}

@inproceedings{CIFAR10,
  title={Learning Multiple Layers of Features from Tiny Images},
  author={A. Krizhevsky},
  year={2009}
}

@INPROCEEDINGS{Imagenet,
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},
  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={ImageNet: A large-scale hierarchical image database}, 
  year={2009},
  volume={},
  number={},
  pages={248-255},
  doi={10.1109/CVPR.2009.5206848}}
  
@techreport{cub,
	Author = {P. Welinder and S. Branson and T. Mita and C. Wah and F. Schroff and S. Belongie and P. Perona},
	Institution = {California Institute of Technology},
	Number = {CNS-TR-2010-001},
	Title = {{Caltech-UCSD Birds 200}},
	Year = {2010}
}

@article{resnet,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Deep Residual Learning for Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1512.03385},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03385},
  archivePrefix = {arXiv},
  eprint    = {1512.03385},
  timestamp = {Wed, 17 Apr 2019 17:23:45 +0200},
}

@inproceedings{SVHN,
  title={Reading Digits in Natural Images with Unsupervised Feature Learning},
  author={Yuval Netzer and T. Wang and A. Coates and A. Bissacco and B. Wu and A. Ng},
  year={2011}
}


@article{pseudolabel,
author = {Lee, Dong-Hyun},
year = {2013},
month = {07},
pages = {},
title = {Pseudo-Label : The Simple and Efficient Semi-Supervised Learning Method for Deep Neural Networks},
journal = {ICML 2013 Workshop : Challenges in Representation Learning (WREPL)}
}

@misc{VAT,
      title={Virtual Adversarial Training: A Regularization Method for Supervised and Semi-Supervised Learning}, 
      author={Takeru Miyato and Shin-ichi Maeda and Masanori Koyama and Shin Ishii},
      year={2018},
      eprint={1704.03976},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}



@article{SWA,
  author    = {Ben Athiwaratkun and
               Marc Finzi and
               Pavel Izmailov and
               Andrew Gordon Wilson},
  title     = {Improving Consistency-Based Semi-Supervised Learning with Weight Averaging},
  journal   = {CoRR},
  volume    = {abs/1806.05594},
  year      = {2018},
  url       = {http://arxiv.org/abs/1806.05594},
  archivePrefix = {arXiv},
  eprint    = {1806.05594},
  timestamp = {Mon, 13 Aug 2018 16:46:09 +0200},
}





@article{uasd,
author = {Chen, Yanbei and Zhu, Xiatian and Li, Wei and Gong, Shaogang},
year = {2020},
month = {04},
pages = {3569-3576},
title = {Semi-Supervised Learning under Class Distribution Mismatch},
volume = {34},
journal = {Proceedings of the AAAI Conference on Artificial Intelligence},
doi = {10.1609/aaai.v34i04.5763}
}

@article{RealMix,
  author    = {Varun Nair and
               Javier Fuentes Alonso and
               Tony Beltramelli},
  title     = {RealMix: Towards Realistic Semi-Supervised Deep Learning Algorithms},
  journal   = {CoRR},
  volume    = {abs/1912.08766},
  year      = {2019},
  url       = {http://arxiv.org/abs/1912.08766},
  archivePrefix = {arXiv},
  eprint    = {1912.08766},
  timestamp = {Fri, 03 Jan 2020 16:10:45 +0100},
}


@article{van2020survey,
  title={A survey on semi-supervised learning},
  author={Van Engelen, Jesper E and Hoos, Holger H},
  journal={Machine Learning},
  volume={109},
  number={2},
  pages={373--440},
  year={2020},
  publisher={Springer}
}

@inproceedings{s4l,
  title={S4l: Self-supervised semi-supervised learning},
  author={Zhai, Xiaohua and Oliver, Avital and Kolesnikov, Alexander and Beyer, Lucas},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1476--1485},
  year={2019}
}

@article{mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin},
  journal={arXiv preprint arXiv:1905.02249},
  year={2019}
}


@article{selflabelsurvey,
author = {Triguero, Isaac and Garc\'{\i}a, Salvador and Herrera, Francisco},
title = {Self-Labeled Techniques for Semi-Supervised Learning: Taxonomy, Software and Empirical Study},
year = {2015},
issue_date = {February  2015},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
volume = {42},
number = {2},
issn = {0219-1377},
journal = {Knowl. Inf. Syst.},
month = feb,
pages = {245–284},
}


@article{sohn2020simple,
  title={A simple semi-supervised learning framework for object detection},
  author={Sohn, Kihyuk and Zhang, Zizhao and Li, Chun-Liang and Zhang, Han and Lee, Chen-Yu and Pfister, Tomas},
  journal={arXiv preprint arXiv:2005.04757},
  year={2020}
}

@inproceedings{arazo2020pseudo,
  title={Pseudo-labeling and confirmation bias in deep semi-supervised learning},
  author={Arazo, Eric and Ortego, Diego and Albert, Paul and O’Connor, Noel E and McGuinness, Kevin},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}

@article{rizve2021defense,
  title={In defense of pseudo-labeling: An uncertainty-aware pseudo-label selection framework for semi-supervised learning},
  author={Rizve, Mamshad Nayeem and Duarte, Kevin and Rawat, Yogesh S and Shah, Mubarak},
  journal={arXiv preprint arXiv:2101.06329},
  year={2021}
}

@inproceedings{lokhande2020generating,
  title={Generating accurate pseudo-labels in semi-supervised learning and avoiding overconfident predictions via Hermite polynomial activations},
  author={Lokhande, Vishnu Suresh and Tasneeyapant, Songwong and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11435--11443},
  year={2020}
}


@inproceedings{simclr,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@inproceedings{moco,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9729--9738},
  year={2020}
}


@article{simclr-v2,
  title={Big Self-Supervised Models are Strong Semi-Supervised Learners},
  author={Chen, Ting and Kornblith, Simon and Swersky, Kevin and Norouzi, Mohammad and Hinton, Geoffrey},
  journal={arXiv preprint arXiv:2006.10029},
  year={2020}
}


@article{kim2021selfmatch,
  title={SelfMatch: Combining Contrastive Self-Supervision and Consistency for Semi-Supervised Learning},
  author={Kim, Byoungjip and Choo, Jinho and Kwon, Yeong-Dae and Joe, Seongho and Min, Seungjai and Gwon, Youngjune},
  journal={arXiv preprint arXiv:2101.06480},
  year={2021}
}


@inproceedings{rasmus2015semi,
  title={Semi-supervised learning with Ladder networks},
  author={Rasmus, Antti and Valpola, Harri and Honkala, Mikko and Berglund, Mathias and Raiko, Tapani},
  booktitle={Proceedings of the 28th International Conference on Neural Information Processing Systems-Volume 2},
  pages={3546--3554},
  year={2015}
}

@inproceedings{bachman2014learning,
  title={Learning with pseudo-ensembles},
  author={Bachman, Philip and Alsharif, Ouais and Precup, Doina},
  booktitle={Proceedings of the 27th International Conference on Neural Information Processing Systems-Volume 2},
  pages={3365--3373},
  year={2014}
}


@inproceedings{TemporalEnsembling,
  title={Temporal ensembling for semi-supervised learning},
  author={Laine, Samuli and Aila, Timo},
  booktitle={International Conference on Learning Representations},
  year={2016}
}

@inproceedings{tarvainen2017mean,
  title={Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
  author={Tarvainen, Antti and Valpola, Harri},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={1195--1204},
  year={2017}
}


@article{miyato2018virtual,
  title={Virtual adversarial training: a regularization method for supervised and semi-supervised learning},
  author={Miyato, Takeru and Maeda, Shin-ichi and Koyama, Masanori and Ishii, Shin},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={8},
  pages={1979--1993},
  year={2018},
  publisher={IEEE}
}


@inproceedings{verma2019interpolation,
 author = {Verma, Vikas and Lamb, Alex and Kannala, Juho and Bengio, Yoshua and Lopez-Paz, David},
 title = {Interpolation Consistency Training for Semi-supervised Learning},
 booktitle = {Proceedings of the 28th International Joint Conference on Artificial Intelligence},
 series = {IJCAI'19},
 year = {2019},
} 



@article{le2015tiny,
  title={Tiny imagenet visual recognition challenge},
  author={Le, Ya and Yang, Xuan},
  journal={CS 231N},
  volume={7},
  pages={7},
  year={2015}
}

@article{ben2007analysis,
  title={Analysis of representations for domain adaptation},
  author={Ben-David, Shai and Blitzer, John and Crammer, Koby and Pereira, Fernando and others},
  journal={Advances in neural information processing systems},
  volume={19},
  pages={137},
  year={2007},
  publisher={MIT; 1998}
}

@inproceedings{panareda2017open,
  title={Open set domain adaptation},
  author={Panareda Busto, Pau and Gall, Juergen},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={754--763},
  year={2017}
}

@inproceedings{saito2018open,
  title={Open set domain adaptation by backpropagation},
  author={Saito, Kuniaki and Yamamoto, Shohei and Ushiku, Yoshitaka and Harada, Tatsuya},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={153--168},
  year={2018}
}

@inproceedings{liu2019separate,
  title={Separate to adapt: Open set domain adaptation via progressive separation},
  author={Liu, Hong and Cao, Zhangjie and Long, Mingsheng and Wang, Jianmin and Yang, Qiang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2927--2936},
  year={2019}
}


@inproceedings{mpl,
  title={Meta pseudo labels},
  author={Pham, Hieu and Dai, Zihang and Xie, Qizhe and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11557--11568},
  year={2021}
}


@article{uda,
  title={Unsupervised Data Augmentation for Consistency Training},
  author={Xie, Qizhe and Dai, Zihang and Hovy, Eduard and Luong, Thang and Le, Quoc},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}

@article{mixup,
  author    = {Hongyi Zhang and
               Moustapha Ciss{\'{e}} and
               Yann N. Dauphin and
               David Lopez{-}Paz},
  title     = {mixup: Beyond Empirical Risk Minimization},
  journal   = {CoRR},
  volume    = {abs/1710.09412},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.09412},
  archivePrefix = {arXiv},
  eprint    = {1710.09412},
  timestamp = {Mon, 13 Aug 2018 16:47:14 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1710-09412.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{remixmatch,
  author    = {David Berthelot and
               Nicholas Carlini and
               Ekin D. Cubuk and
               Alex Kurakin and
               Kihyuk Sohn and
               Han Zhang and
               Colin Raffel},
  title     = {ReMixMatch: Semi-Supervised Learning with Distribution Alignment and
               Augmentation Anchoring},
  journal   = {CoRR},
  volume    = {abs/1911.09785},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.09785},
  archivePrefix = {arXiv},
  eprint    = {1911.09785},
  timestamp = {Wed, 03 Feb 2021 15:07:57 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-09785.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{oliver,
  author    = {Avital Oliver and
               Augustus Odena and
               Colin Raffel and
               Ekin D. Cubuk and
               Ian J. Goodfellow},
  title     = {Realistic Evaluation of Deep Semi-Supervised Learning Algorithms},
  journal   = {CoRR},
  volume    = {abs/1804.09170},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.09170},
  archivePrefix = {arXiv},
  eprint    = {1804.09170},
  timestamp = {Mon, 13 Aug 2018 16:46:38 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-09170.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@InProceedings{ds3l,
  title = 	 {Safe Deep Semi-Supervised Learning for Unseen-Class Unlabeled Data},
  author =       {Guo, Lan-Zhe and Zhang, Zhen-Yu and Jiang, Yuan and Li, Yu-Feng and Zhou, Zhi-Hua},
  booktitle = 	 {Proceedings of the 37th International Conference on Machine Learning},
  pages = 	 {3897--3906},
  year = 	 {2020},
  editor = 	 {III, Hal Daumé and Singh, Aarti},
  volume = 	 {119},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {13--18 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v119/guo20i/guo20i.pdf},
  url = 	 {http://proceedings.mlr.press/v119/guo20i.html},
}

@article{jigsaw,
  author    = {Mehdi Noroozi and
               Paolo Favaro},
  title     = {Unsupervised Learning of Visual Representations by Solving Jigsaw
               Puzzles},
  journal   = {CoRR},
  volume    = {abs/1603.09246},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.09246},
  archivePrefix = {arXiv},
  eprint    = {1603.09246},
  timestamp = {Mon, 13 Aug 2018 16:49:09 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/NorooziF16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{wrn,
  author    = {Sergey Zagoruyko and
               Nikos Komodakis},
  title     = {Wide Residual Networks},
  journal   = {CoRR},
  volume    = {abs/1605.07146},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.07146},
  archivePrefix = {arXiv},
  eprint    = {1605.07146},
  timestamp = {Mon, 13 Aug 2018 16:46:42 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ZagoruykoK16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{banitalebi2021knowledge,
  title={Knowledge distillation for low-power object detection: A simple technique and its extensions for training compact models using unlabeled data},
  author={Banitalebi-Dehkordi, Amin},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={769--778},
  year={2021}
}


@article{banitalebi2021revisiting,
  title={Revisiting Knowledge Distillation for Object Detection},
  author={Banitalebi-Dehkordi, Amin},
  journal={arXiv preprint arXiv:2105.10633},
  year={2021}
}


@inproceedings{banitalebi2021repaint,
  title={Repaint: Improving the Generalization of Down-Stream Visual Tasks by Generating Multiple Instances of Training Examples},
  author={Banitalebi-Dehkordi, Amin and Zhang, Yong},
  booktitle={the 32nd British Machine Vision Conference},
year={2021}
}

@inproceedings{ramamonjison2021simrod,
  title={Simrod: A simple adaptation method for robust object detection},
  author={Ramamonjison, Rindra and Banitalebi-Dehkordi, Amin and Kang, Xinyu and Bai, Xiaolong and Zhang, Yong},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3570--3579},
  year={2021}
}



